The ELBO of Variational Autoencoders Converges to a Sum of Three Entropies

The central objective function of a variational autoencoder (VAE) is its variational lower bound (the ELBO). Here we show that for standard (i.e., Gaussian) VAEs the ELBO converges to a value given by the sum of three entropies: the (negative) entropy of the prior distribution, the expected (negative) entropy of the observable distribution, and the average entropy of the variational distributions (the latter is already part of the ELBO). Our derived analytical results are exact and apply for small as well as for intricate deep networks for encoder and decoder. Furthermore, they apply for finitely and infinitely many data points and at any stationary point (including local maxima and saddle points). The result implies that the ELBO can for standard VAEs often be computed in closed-form at stationary points while the original ELBO requires numerical approximations of integrals. As a main contribution, we provide the proof that the ELBO for VAEs is at stationary points equal to entropy sums. Numerical experiments then show that the obtained analytical results are sufficiently precise also in those vicinities of stationary points that are reached in practice. Furthermore, we discuss how the novel entropy form of the ELBO can be used to analyze and understand learning behavior. More generally, we believe that our contributions can be useful for future theoretical and practical studies on VAE learning as they provide novel information on those points in parameters space that optimization of VAEs converges to.

==> figs/Code.tex <==
\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\ttfamily\footnotesize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=t,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2,
		frame=lines,
		language=Python,
}

\lstset{style=mystyle}
\lstset{caption={Example Implementations}}
\lstset{label={lst:Code}}
\begin{lstlisting}
import torch
from torch.nn import Linear, Module, Parameter
from torch.nn.functional import softplus
from torch.distributions import Normal, kl_divergence
import math
pi = torch.Tensor([math.pi])

class LinearVAE(Module):
    def __init__(self, H, D, num_samples=100):
        super(LinearVAE, self).__init__()
        self.H = H
        self.D = D
        self.num_samples = num_samples

        self.encoder = Linear(D, H)
        self.decoder = Linear(H, D)
        self.noise_std = Parameter(torch.Tensor([0.]))
        self.q_z_std = Parameter(torch.zeros(H))
        self.p_z = Normal(torch.Tensor([0.]), torch.Tensor([1.]))

    def forward(self, x):
        sigma = softplus(self.noise_std)
        tau = softplus(self.q_z_std)
        N, D = x.shape

        z_params = self.encoder(x)
        q_z = Normal(z_params, tau)

        z_samples = q_z.rsample([self.num_samples])
        p_x_z_mean = self.decoder(z_samples)
        p_x_z = Normal(p_x_z_mean, sigma)

        lower_bound = p_x_z.log_prob(x).mean(0).sum() \
                      - kl_divergence(q_z, self.p_z).sum()
        three_entropies_linear = self.three_entropies_linear(N, D, sigma, tau)
        return lower_bound, three_entropies_linear

    @staticmethod
    def three_entropies_linear(N, D, sigma, tau):
        """Three Entropies (accumulated) for linear VAE, Eq.(33).
        Args:
            N (int) : batch size
            D (int) : output dimensionality
            sigma (torch.tensor, size=(1,)) : decoder standard deviation
            tau (torch.tensor, size=(H,)    : encoder standard deviation
        """
        return N*(-D/2*(torch.log(2*pi)+1)-D*torch.log(sigma)+torch.log(tau).sum())

class VAE1(Module):
		
		[...]		

    @staticmethod
    def three_entropies_nonlinear(N, D, sigma, tau):
        """Three Entropies (accumulated) for non-linear VAE (VAE-1), Eq.(25).
        Args:
            N (int) : batch size
            D (int) : output dimensionality
            sigma (torch.tensor, size=(1,)) : decoder standard deviation
            tau (torch.tensor, size=(N, H)) : encoder standard deviation
        """
        return N*D*(-1/2*(torch.log(2*pi)+1)-torch.log(sigma)) + torch.log(tau).sum()

class VAE3(Module):
		
		[...]
		
		@staticmethod
    def three_entropies_sigmaz(N, D, sigma, tau):
        """Three Entropies (accumulated) for sigma(z)-VAE (VAE-3), Eq.(39).
        Args:
            N (int) : batch size
            D (int) : output dimensionality
            sigma (torch.tensor, size=(num_samples, N, D)) : decoder std
            tau (torch.tensor, size=(N, H)) : encoder standard deviation
        """
        return -N*D/2*(torch.log(2*pi)+1) - torch.log(sigma).mean(0).sum() \
				       + torch.log(tau).sum()
\end{lstlisting}


==> figs/Fig3.tex <==
\begin{wrapfigure}{r}{5.5cm}
\vspace{-6pt}
  \centering
  \includegraphics[width=5.5cm]{figs/Fig3a.pdf}  
\vspace{-14pt}
\caption{\todo{Correlation between lower bound and three entropies of \mbox{VAE--3} on the same PCA-ring data set over 100~runs. A pearson correlation coefficient (PCC) of +1 would indicate total positive linear correlation.}}
\label{fig:correlation}
\vspace{-22pt}
\end{wrapfigure}

